BudgetFusion: Perceptually-Guided Adaptive Diffusion Models

Diffusion models have shown unprecedented success in the task of text-to-image generation. While these models are capable of generating high-quality and realistic images, the complexity of sequential denoising has raised societal concerns regarding high computational demands and energy consumption. In response, various efforts have been made to improve inference efficiency. However, most of the existing efforts have taken a fixed approach with neural network simplification or text prompt optimization. Are the quality improvements from all denoising computations equally perceivable to humans? We observed that images from different text prompts may require different computational efforts given the desired content. The observation motivates us to present BudgetFusion, a novel model that suggests the most perceptually efficient number of diffusion steps before a diffusion model starts to generate an image. This is achieved by predicting multi-level perceptual metrics relative to diffusion steps. With the popular Stable Diffusion as an example, we conduct both numerical analyses and user studies. Our experiments show that BudgetFusion saves up to five seconds per prompt without compromising perceptual similarity. We hope this work can initiate efforts toward answering a core question: how much do humans perceptually gain from images created by a generative model, per watt of energy?

==> Makefile <==
TARGETS    = targets
BUILD      = build

.PHONY: all internal submission revision camready camauthor clean

all: internal submission revision camready camauthor

internal:   $(BUILD)/internal.manuscript.compressed.pdf\
            $(BUILD)/internal.supplement.compressed.pdf\
	    $(BUILD)/internal.all.compressed.pdf

submission: $(BUILD)/submission.manuscript.compressed.pdf\
            $(BUILD)/submission.supplement.compressed.pdf\
	    $(BUILD)/submission.all.compressed.pdf

revision:   $(BUILD)/revision.manuscript.compressed.pdf\
            $(BUILD)/revision.supplement.compressed.pdf\
	    $(BUILD)/revision.all.compressed.pdf

camready:   $(BUILD)/camready.manuscript.compressed.pdf\
            $(BUILD)/camready.supplement.compressed.pdf\
	    $(BUILD)/camready.all.compressed.pdf

camauthor:  $(BUILD)/camauthor.manuscript.compressed.pdf\
            $(BUILD)/camauthor.supplement.compressed.pdf\
	    $(BUILD)/camauthor.all.compressed.pdf

%.compressed.pdf : %.pdf
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.5 -dNOPAUSE -dQUIET -dBATCH -dPrinted=false -sOutputFile=$*.compressed.pdf $*.pdf

%.supplement.pdf : %.manuscript.pdf %.all.pdf
	gs -dNOPAUSE -dQUIET -dBATCH -sOutputFile="$*.supplement.pdf" -dFirstPage=$$(echo $$(gs -q -dNODISPLAY -dNOSAFER -c "($*.manuscript.pdf) (r) file runpdfbegin pdfpagecount = quit") + 1 | bc) -dLastPage=$$(gs -q -dNODISPLAY -dNOSAFER -c "($*.all.pdf) (r) file runpdfbegin pdfpagecount = quit") -sDEVICE=pdfwrite "$*.all.pdf"

%.manuscript.pdf : %.all.pdf
	# Make manuscript version of paper.tex
	cat $(TARGETS)/$(*F).tex | sed 's/\\\input{paper}/\\\input{paper.manuscript}/' > $(TARGETS)/$(*F).manuscript.tex
	# First generate support files
	cat paper.tex | sed 's/^.*\\\includeonly{}/% \\\includeonly{}/' > paper.manuscript.tex
	pdflatex -jobname=$*.manuscript $(TARGETS)/$(*F).manuscript.tex
	# Remove supplement section
	cat paper.tex | sed 's/^.*\\\includeonly{}/\\\includeonly{}/' > paper.manuscript.tex
	pdflatex -jobname=$*.manuscript $(TARGETS)/$(*F).manuscript.tex
	bibtex $*.manuscript.aux
	pdflatex -jobname=$*.manuscript $(TARGETS)/$(*F).manuscript.tex
	pdflatex -jobname=$*.manuscript $(TARGETS)/$(*F).manuscript.tex
	# Clean-up temporary files
	rm -f paper.manuscript.tex $(TARGETS)/$(*F).manuscript.tex

%.all.pdf :
	mkdir -p $(BUILD)
	pdflatex -jobname=$*.all $(TARGETS)/$(*F).tex
	bibtex $*.all.aux
	pdflatex -jobname=$*.all $(TARGETS)/$(*F).tex
	pdflatex -jobname=$*.all $(TARGETS)/$(*F).tex

clean:
	rm -rf $(BUILD)


==> conf/packages.tex <==
%%% Language %%%%
\RequirePackage[english]{babel}                  % Hyphenation and date format
\RequirePackage{xspace}                          % Abbreviation spacing
\RequirePackage{xpunctuate}                      % Abbreviation spacing

%%% Tex-scripting %%%
\RequirePackage{ifthen}                          % If-then-else latex logic
\RequirePackage{soul}                            % Underlining and Strike-through
\RequirePackage{xargs}                           % For \newcommandx

%%% Color %%%
\RequirePackage{color}                           % Draft annotation coloring

%%% Math-mode %%%
\RequirePackage{amsmath}                         % Math equations
\RequirePackage{bm}                              % Math bold symbols

%%% Cross-referencing %%%
\RequirePackage[toc,page,titletoc]{appendix}     % Appendix section
\RequirePackage[capitalize,nameinlink]{cleveref} % Easy to use cross-referencing
\crefname{supp}{Supplement}{Supplements}     % Supplement section name setting

%%% Figures %%%
\RequirePackage{caption}                         % Figure captions
%\RequirePackage{subfig}                          % Nested figures

\usepackage{enumitem}

==> content/frontmatter/acks.tex <==
To Robert, for the bagels and explaining CMYK and color spaces.

==> figures/denoising_step_images.tex <==
\begin{figure}
\centering
% \subfloat[step x]{
%     \includegraphics[width=0.32\linewidth]{example-image-a}
%   }
\subfloat[step y]{
    \includegraphics[width=0.32\linewidth]{example-image-a}
  }
\subfloat[step z]{
    \includegraphics[width=0.32\linewidth]{example-image-a}
  }  
\includegraphics[width=\linewidth]{assets/efficient-diffusion-example.pdf}
\Caption{Example of images generated with different steps of text prompt ``xxxxxxxx''.}
{
}
\Description{}
\label{fig:method:steps}
\end{figure}

==> figures/detailed_user_study.tex <==
\begin{figure}
  \centering
  \includegraphics[width=.9\linewidth]{assets/efficient-diffusion-per-scene-study.pdf}
  \Caption{
      Per-scene user study results.
  }{
    % \warning{In the appendix we could add a table of per-user responses as well as the stimuli used in the study.}
    %\warning{add the timestep for each image?}
    We include the user study results averaged across scenes (right column), including the text prompt used to generate each image, as well as the generated images for all three conditions.
  }
  \label{fig:study:all}
   \label{fig:study:byscene}
\Description{}
\end{figure}


==> figures/teaser.tex <==
\begin{teaserfigure}
\centering
\includegraphics[width=\linewidth]{assets/efficient-diffusion-teaser.pdf}
\Caption{Guiding perceptually-efficient denoising steps for pre-trained diffusion model.}{
Given an input text prompt, our \methodName model guides the number of denoising steps $\step$ before the generation starts.  It balances the trade-off between visual perception quality and computational cost, achieving an optimized ``quality gain per denoising step'' efficiency.
%, during inference of a pre-trained diffusion model, which generates perceptually-optimal images.
%That is, it optimizes the diffusion efficiency as ``quality gain per timestep''.
}
\label{fig:teaser}
\Description{}
\end{teaserfigure}


==> metadata/acm/index.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010371.10010387.10010866</concept_id>
<concept_desc>Computing methodologies~Virtual reality</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010371.10010387.10010392</concept_id>
<concept_desc>Computing methodologies~Mixed / augmented reality</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010371.10010387.10010393</concept_id>
<concept_desc>Computing methodologies~Perception</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010257.10010293.10010294</concept_id>
<concept_desc>Computing methodologies~Neural networks</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Artificial intelligence}
\ccsdesc[500]{Computing methodologies~Perception}
\ccsdesc[500]{Computing methodologies~Neural networks}

\keywords{Visual perception, Generative models}

==> metadata/acm/paper.tex <==
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
%% \title[short title]{full title}
%% Capitalize your title: https://capitalizemytitle.com/
%\title{A method for predicting text-adaptive inference steps for Stable Diffusion}

\title[\methodName]{\methodName: Perceptually-Guided Low-Power Optimization for Generative Models}
\title[\methodName]{\methodName: Perceptually-Guided Computation Optimization for Generative Models}
\title[\methodName]{\methodName: Perceptually-Guided Generative Models for Low-Power Computation}
\title[\methodName]{\methodName: Towards Low-Power Generative Models Guided by Visual Perception}
\title[\methodName]{\methodName: Perceptually-Guided Low-Power Generative Models}

\title[\methodName]{\methodName: Perceptually-Guided Adaptive Diffusion Models}

%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.

\author{anonymous authors}

% \author{Qinchan(Wing) Li}
% \email{ql840@nyu.edu}
% \orcid{1234-5678-9012}
% \authornotemark[1]
% \affiliation{%
%   \institution{New York University}
%   \streetaddress{P.O. Box 1212}
%   \city{New York}
%   \state{New York}
%   \country{USA}
%   \postcode{43017-6221}
% }



% \author{Kenneth Chen}

% \email{kc4906@nyu.edu}
% \affiliation{%
%   \institution{New York University}
%   \streetaddress{P.O. Box 1212}
%   \city{New York}
%   \state{New York}
%   \country{USA}
%   \postcode{43017-6221}
% }

% \author{Qi Sun}

% \email{qisun@nyu.edu}
% \affiliation{%
%   \institution{New York University}
%   \streetaddress{P.O. Box 1212}
%   \city{New York}
%   \state{New York}
%   \country{USA}
%   \postcode{43017-6221}
% }

%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
%\renewcommand{\shortauthors}{Trovato and Tobin, et al.}


==> metadata/acm/tog.tex <==
\setcopyright{acmcopyright}
\copyrightyear{2022}
\acmJournal{TOG}
\acmYear{2022}
\acmVolume{41}
\acmNumber{6}
\acmArticle{1}
\acmDOI{}
\acmSubmissionID{625}
\citestyle{acmauthoryear}


==> metadata/dissertate/paper.tex <==
% Some details about the dissertation.
\title{Psychophysical Methods for Enhancing Immersive Graphics Systems}
\author{Budmonde Duinkharjav}
\advisor{Qi Sun}

% ... about the degree.
\degree{Doctor of Philosophy}
\field{Computer Science}
\degreeyear{2024}
\degreemonth{May}
\department{Computer Science and Engineering}

% ... about the candidate's previous degrees.
\pdOneName{B.S.}
\pdOneSchool{Massachusetts Institute of Techology}
\pdOneYear{2018}

\pdOneName{M.Eng.}
\pdOneSchool{Massachusetts Institute of Techology}
\pdOneYear{2019}

==> tables/tab_quality.tex <==
\begin{table}
\captionsetup{aboveskip=1.0ex}
    \caption{Quality gain ratio across all prompts.}
    \label{tab:qualityRatio}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lrrr}
        \toprule
        Model & \SNRLaplacian  & \dreamsim  & \clip  \\
        \midrule
        \condOurs & $3.6\text{e-}3\pm 3.8\text{e-}5$  & $1.95\text{e-}2\pm 1.2\text{e-}4$ & $1.0\text{e-}2\pm 6.5\text{e-}5$  \\ 
        % \hline
        \condUniform & $3.5\text{e-}3\pm 3.1\text{e-}5$ & $1.86\text{e-}2\pm 3.9\text{e-}5$  & $0.97\text{e-}2\pm 2.8\text{e-}5$  \\
        \bottomrule
    \end{tabular}
    }
\end{table}


%Statistically, we acquire $6.6\% \pm 0.8\%$ for $\metric$=\SNRLaplacian, $8.4\% \pm 0.9\%$ for $\metric$=\dreamsim, and $8.7\%\pm0.9\%$ for $\metric$=\clip.
